SmBoP: Semi-autoregressive Bottom-up Semantic Parsing

The de-facto standard decoding method for semantic parsing in recent years has been to autoregressively decode the abstract syntax tree of the target program using a top-down depth-first traversal. In this work, we propose an alternative approach: a Semi-autoregressive Bottom-up Parser (SmBoP) that constructs at decoding step $t$ the top-$K$ sub-trees of height $\leq t$. Our parser enjoys several benefits compared to top-down autoregressive parsing. From an efficiency perspective, bottom-up parsing allows to decode all sub-trees of a certain height in parallel, leading to logarithmic runtime complexity rather than linear. From a modeling perspective, a bottom-up parser learns representations for meaningful semantic sub-programs at each step, rather than for semantically-vacuous partial trees. We apply SmBoP on Spider, a challenging zero-shot semantic parsing benchmark, and show that SmBoP leads to a 2.2x speed-up in decoding time and a $\sim$5x speed-up in training time, compared to a semantic parser that uses autoregressive decoding. SmBoP obtains 71.1 denotation accuracy on Spider, establishing a new state-of-the-art, and 69.5 exact match, comparable to the 69.6 exact match of the autoregressive RAT-SQL+GraPPa.

==> 05_related_work.tex <==
\section{Related Work}
Generative models whose runtime complexity is sub-linear have been explored recently outside semantic parsing.
The Insertion Transformer \cite{stern2019Insertion} is a partially autoregressive model in machine translation, where at each step multiple tokens from the target are generated. Unlike machine translation, in semantic parsing the target is a tree, which induces a particular way to generate sub-trees in parallel. More generally, there has been ample work in machine translation aiming to speed up inference through non-autoregressive or semi-autoregressive generation (\citet{wang2018semiautoregressiveNM,Ghazvininejad2020SemiAutoregressiveTI,Saharia2020NonAutoregressiveMT}; among others).

\mycomment{
In program syntehsis, \newcite{odena2020bustle}
recently proposed a bottom-up parser, where search is improved by executing partial queries and conditioning on the resulting values, similar to  some work in semantic parsing \cite{berant2013freebase,liang2017nsm}. We do not explore this advantage of bottom-up parsing here, since executing queries at training slows it down.
}
